Towards Balanced Behavior Cloning from Imbalanced Datasets

Robots should be able to learn complex behaviors from human demonstrations. In practice, these human-provided datasets are inevitably imbalanced: i.e., the human demonstrates some subtasks more frequently than others. State-of-the-art methods default to treating each element of the human's dataset as equally important. So if -- for instance -- the majority of the human's data focuses on reaching a goal, and only a few state-action pairs move to avoid an obstacle, the learning algorithm will place greater emphasis on goal reaching. More generally, misalignment between the relative amounts of data and the importance of that data causes fundamental problems for imitation learning approaches. In this paper we analyze and develop learning methods that automatically account for mixed datasets. We formally prove that imbalanced data leads to imbalanced policies when each state-action pair is weighted equally; these policies emulate the most represented behaviors, and not the human's complex, multi-task demonstrations. We next explore algorithms that rebalance offline datasets (i.e., reweight the importance of different state-action pairs) without human oversight. Reweighting the dataset can enhance the overall policy performance. However, there is no free lunch: each method for autonomously rebalancing brings its own pros and cons. We formulate these advantages and disadvantages, helping other researchers identify when each type of approach is most appropriate. We conclude by introducing a novel meta-gradient rebalancing algorithm that addresses the primary limitations behind existing approaches. Our experiments show that dataset rebalancing leads to better downstream learning, improving the performance of general imitation learning algorithms without requiring additional data collection. See our project website: https://collab.me.vt.edu/data_curation/.

==> 5_method.tex <==
\section{Balancing the Dataset}

% Tradintional objective leads to bias
% tie to analysis
% from the analysis, the loss for underrepresented sub policies is high, refer to example
% Ideally, data across sub-policies must be 1/k
% So, standard objective is expectation over p
% ideally we want it over q
% if we know the sub policy labels, we can learn how to weigh them, cite remix
% but we don't. So we use our intuition to identify the points that must be upsampled
% discuss method procedure
% algorithm

In the previous section we show that the learned policy is influenced by the joint probability density of the states and actions in the dataset.
If the state-action pairs associated with a sub-policy are more abundant, this sub-policy can \textit{bias} the robot's policy.
To learn a robot policy that can execute each of the human expert's behaviors reliably, we need to uniformly weigh each sub-policy present in the dataset.
To this end, in this section we propose an \textit{unsupervised} approach for curating the dataset such that each sub-policy is weighted uniformly rather than according to their proportion in the dataset.
We start by formally discussing what curating the dataset entails, then we detail our approach for achieving this.


% Below is a sketch of our approach:
% \begin{itemize}
%     \item Given dataset of offline demonstrations $\mathcal{D}$
%     \item Divide dataset into $\mathcal{D}_f$ and $\mathcal{D}_R$. Here $\mathcal{D}_f$ contains state-actions pairs that encode data about the constraint, and $\mathcal{D}_R = \mathcal{D} \setminus \mathcal{D}_f$.
%     \item Create new dataset $\mathcal{D}' \subseteq \mathcal{D}$ by sampling $K_f$ datapoints from $\mathcal{D}_f$ and $K_R$ datapoints from $\mathcal{D}_R$.
%     \item Use standard loss function to train agent on dataset $\mathcal{D}'$
% \end{itemize}

% Heramb Notes:
% From our analysis, we know that for balanced we need to sample according to q(s, a)
% which is equivalent to uniformly sampling from D*
% challenge is that we do not have D* (nor do we know \rho to calculate q -- because we don't have behavior labels)
% But we have D 
% we can use importance sampling with weights w = q/p
% so E_{p} w log \pi
% remember we still don't know q. how do we get it?
% we know from analysis that Error is inversely proportional to \rho, Error \propto (1 - \rho)
% we also know that q = p/\rho, so w is also inversely proportional to \rho
% therefore we consider w \propto Error
% then go through algorithm and talk about implementation in next paragraphs

In standard behavior cloning the objective, given in \eq{P1}, maximizes the expected likelihood of correct actions over the joint state-action distribution $p(s, a)$ in the dataset.
As we showed in the previous section, the sub-policies with greater proportion of samples in the dataset bias the learned policy's parameters.
To counter this bias, we need to update the objective: we maximize the expected likelihood of correct actions over the curated state-action distribution $q(s, a)$.
Recall that the dataset has an underlying distribution $p(s, a)$, which is the joint probability of a state-action pair being in the dataset $\mathcal{D}$.
This joint probability can be skewed since some sub-policies can have more state-action samples than others.
As we show previously, $q(s, a) = \frac{p(s, a)}{\rho_i}$ is the ideal joint probability distribution we must have in order to learn an unbiased policy. Here, $\rho_i$ is the probability associated with the sub-policy $\pi_i$.
Below we compare the standard behavior cloning objective given dataset $\mathcal{D}$ with the ideal objective that we need to optimize to learn an unbiased policy.

\begin{align}
    \text{standard imitation learning objective: } & - \mathop{\mathbb{E}}\limits_{(s, a) \sim p} \log \pi_{\theta}(a | s) \label{eq:M1}\\
    \text{ideal imitation learning objective: } & - \mathop{\mathbb{E}}\limits_{(s, a) \sim q} \log \pi_{\theta}(a | s) \label{eq:M2}
\end{align}

Alternatively, we can say that we are given a dataset $\mathcal{D}$ with underlying probability density $p$ which may have an imbalance between the sub-policies.
We must curate this dataset to get $\mathcal{D}^*$ that has probability density $q$ before learning a robot policy so that we can reliably execute all the behaviors exhibited by the human expert.
Since we do not have $\mathcal{D}^*$, we use importance sampling to emulate sampling state-action pairs from this unknown distribution $q$.
Specifically, we can find a weighting function $w$ for sampling state-action pairs when training the policy $\pi_\theta$ such that it implicitly defines the ideal dataset $\mathcal{D}^*$.
This weighting function is defined as the following ratio 
\begin{equation*}
    w = \frac{q(s, a)}{p(s, a)}
\end{equation*}
With this weighting function, the ideal imitation learning objective becomes
\begin{equation}
    \mathop{\mathbb{E}}\limits_{(s, a) \sim \mathcal{D}^*} \log \pi_\theta (a|s) \approx \mathop{\mathbb{E}}\limits_{(s, a) \sim \mathcal{D}} w \log \pi_\theta (a|s)
\end{equation}

% how previous works do it and what do they need to achieve that
% we don't have access to the same information
% so how do we get the weighting function?
% instead of estimating the weights, we directly estimate the balanced dataset D*
% we leverage our intuition that policy will perform poorly on other sub-policy' states
% upsample the ones with larger error

How do we determine the weighting function $w$?
We refer back to our analysis where we show that (a) a policy trained on an imbalanced dataset is biased, and (b) this biased policy incurs a higher loss on the state-action pairs associated with the minor sub-policies.
Given this, we can use a trained policy to identify the states and actions which correspond to the minor sub-policies.
Particularly, when we train a policy on the given dataset, it is likely to predict inaccurate actions in states where the human uses a sub-policy which is under-represented in the dataset $\mathcal{D}$.
In our example, the policy trained on the imbalanced dataset can accurately predict wiping actions in states that are far away from the cup, but in states closer to the cup the policy might struggle predicting actions that avoid the cup.
Therefore, we can use the prediction error of the trained policy to approximate sampling from 
Therefore, we can use the prediction loss of the biased policy to evaluate state-action pairs and approximate the weighting function using the prediction loss.
Based on the weighting function we can upsample the states and actions to estimate the ideal balanced dataset $\mathcal{D}^*$.

An outline of our approach is presented in \ref{alg:main}.
Given the dataset $\mathcal{D}$, we split it into training and validation sets. 
Using the training set, we train a reference robot policy $\pi_\theta$ using standard imitation learning.
Since, $\mathcal{D}$ is imbalanced, we would expect $\pi_theta$ to be biased by the dominant sub-policies.
We evaluate $\pi_theta$ on the validation set and calculate the mean squared error for the predicted actions. 
We calculate the weighting function as proportional to the prediction error on each state-action pair, i.e., $w \propto \mid\mid \pi_\theta(s) - a \mid\mid$, and upsample the states and actions using this sampling weight.
All the transitions that have a higher prediction error are highly likely to lie outside the underlying distribution of the learned policy.
Remember, the learned policy tries to match the distribution of the dominant sub-policies.
So, these transitions are likely to correspond to the minor sub-policies in the dataset $\mathcal{D}$.
We repeat these steps until convergence, i.e., until the total number of transitions separated by our approach exceeds a predefined threshold.
Following this procedure allows us to upsample the transitions that the policy would struggle with and estimate a balanced dataset $\mathcal{D}^*$.
Finally, we can use $\mathcal{D}^*$ to train a robot policy that learns uniformly learns all the behaviors present in the original dataset.


% \begin{algorithm} \label{alg:main}
%     \caption{Our Method}
%     \begin{algorithmic}
%         \REQUIRE A dataset of state-action pairs $\mathcal{D} = \{(s^1, a^1), \cdots, (s^n, a^n)\}$
%         \REQUIRE Error threshold $\epsilon$ and convergence threshold $\eta$
%         \STATE Initialize an empty set $\Bar{\mathcal{D}} = \emptyset$
%         \WHILE{True}
%             \STATE Initialize counter $i = 0$
%             \STATE Initialize behavior cloning policy $\pi_{\theta}$ with parameters $\theta$
%             \STATE Split the dataset $\Bar{\mathcal{D}} \cup \mathcal{D}$ into train and test sets $\mathcal{D}_{train}$, $\mathcal{D}_{test}$
%             \STATE Train $\pi_{\theta}$ on set $\mathcal{D}_{train}$
%             \FOR{$(s^i, a^i) \in \mathcal{D}_{test}$}
%                 \STATE Find prediction error of the policy $e = \mid\mid \pi_{\theta}(s^i) - a^i \mid\mid$
%                 \IF{$e > \epsilon$}
%                     \STATE $\Bar{\mathcal{D}} \leftarrow \Bar{\mathcal{D}} \cup \{(s^i, a^i)\}$
%                     \STATE $i \leftarrow i + 1$
%                 \ENDIF
%                 \ENDFOR
%             \IF{$i < \eta$}
%                 \STATE \textbf{break}
%             \ENDIF
%         \ENDWHILE

%         \STATE Train behavior cloning policy $\pi_\phi$ with parameters $\phi$ on balanced dataset $\mathcal{D} \cup \Bar{\mathcal{D}}$
%     \end{algorithmic}
% \end{algorithm}
\begin{algorithm} \label{alg:main}
    \caption{Our Method}
    \begin{algorithmic}
        \REQUIRE A dataset of state-action pairs $\mathcal{D} = \{(s^1, a^1), \cdots, (s^n, a^n)\}$
        \REQUIRE Convergence threshold $\eta$
        \STATE Initialize an empty set $\Bar{\mathcal{D}} = \emptyset$
        \WHILE{True}
            \STATE Initialize behavior cloning policy $\pi_{\theta}$ with parameters $\theta$
            \STATE Split the dataset $\Bar{\mathcal{D}} \cup \mathcal{D}$ into train and test sets $\mathcal{D}_{train}$, $\mathcal{D}_{test}$
            \STATE Train $\pi_{\theta}$ on set $\mathcal{D}_{train}$
            \FOR{$(s^i, a^i) \in \mathcal{D}_{test}$}
                \STATE Find prediction error of the policy $e = \mid\mid \pi_{\theta}(s^i) - a^i \mid\mid$
                \ENDFOR
            \STATE Calculate importance weight $w \propto e$
            \STATE Upsample $(s, a)$ based on importance weight $w$ and add to $\Bar{D}$
            \IF{length of $\Bar{D} < \eta$}
                \STATE \textbf{break}
            \ENDIF
        \ENDWHILE
        \STATE Train behavior cloning policy $\pi_\phi$ with parameters $\phi$ on balanced dataset $\mathcal{D} \cup \Bar{\mathcal{D}}$
    \end{algorithmic}
\end{algorithm}

% tie this to your analsis
% basically forces alpha to be uniform (0.5)






% \subsection{Importance Sampling Notes}

% Importance sampling (IS) refers to a collection of Monte Carlo methods
% where a mathematical expectation with respect to a target distribution
% is approximated by a weighted average of random draws from another
% distribution.
% - The "expectation" we want is the expected loss for model weights $\theta$
% - The target distribution is a balanced distribution
% - The "other distribution" is our given, biased dataset
% - The "weighted average" refers to how we increase the weight (i.e., the number of times we check) the loss on the underrepresented points.
% Conclusion: what we are doing is importance sampling.

% we are trying to compute the expected loss for model weights $\theta$
% to do this, we sample state-action pairs from the dataset
% Ideally, we would sample the state-action pairs with probability p, so that the expected loss is:
% \begin{equation}
%     L(\theta) = \mathbb{E}_{(s, a) \sim p} ~L(s, a, \theta)
% \end{equation}
% Here p is an unbiased distribution (i.e., it samples each "type" of data the same amount)
% this means that some (s,a) pairs are more likely to be sampled than others (the ones we sample more are the underrepresented state-action pairs)
% in terms of the analysis, for p each \alpha_i is equal

% But current methods do not do this. Instead, they compute the expected loss under distribution q:
% \begin{equation}
%     L(\theta) = \mathbb{E}_{(s, a) \sim q} ~L(s, a, \theta)
% \end{equation}
% where q just matches the dataset. In other words, under q each (s, a) pair in the original dataset is equally likely of being sampled.
% in terms of the analysis, for q alpha_i is proportional to the number of samples from that type

% So if we are given q, how do we go about finding the expected loss with respect to x?
% here we can use importance sampling
% the basic idea is:
% \begin{equation}
%     L(\theta) = \mathbb{E}_{(s, a) \sim q} ~\frac{p(s,a)}{q(s,a)}L(s, a, \theta)
% \end{equation}
% where p(s,a) is the probability of the state action pair under p, and q is the probability of that same state action pair under q
% this new term is called the "likelihood ratio"
% of course, we don't have a closed form equation to get p/q (because p is unknown a priori, we don't know at the start whether a given state-action pair is part of a common pattern or underrepresented)

% Our method iteratively approximates the likelihood ratio (I think)
% can we prove this? [from here i am just making up stuff]
% maybe we can prove it with the linear regression approach you've already started?
% what you would want to show is that repeatedly taking the state-action pairs with a high loss and upsampling them eventually results in a distribution p where each ai is equal (the classes are uniformly likely)
% probably you could show that numerically first? Like with a simple matlab/python test or something [this is what i recommend doing next]
% I think it should converge to the desired, balanced distribution [because whenever it is unbalanced, one type has higher loss --- meaning we sample them more, so the equilibrium would be when all the losses are equal]
% if so, then we can say that our method iteratively gets the likelihood ratio / performs importance sampling


% should emphasize that the first loss function equation i wrote (wrt p) is really what we want; like that is the premise of our work, we should be using that loss funciton and not the one wrt q.
% this point is sort of like our insight or hypothesis
% because its more based on our logic than any specific rule...






